Scintillation-limited photometry with the 20-cm NGTS telescopes at Paranal Observatory

Ground-based photometry of bright stars is expected to be limited by atmospheric scintillation, although in practice observations are often limited by other sources of systematic noise. We analyse 122 nights of bright star ($G_{mag} < 11.5$) photometry using the 20-cm telescopes of the Next-Generation Transit Survey (NGTS) at the Paranal Observatory in Chile. We compare the noise properties to theoretical noise models and we demonstrate that NGTS photometry of bright stars is indeed limited by atmospheric scintillation. We determine a median scintillation coefficient at the Paranal Observatory of $C_Y = 1.54$, which is in good agreement with previous results derived from turbulence profiling measurements at the observatory. We find that separate NGTS telescopes make consistent measurements of scintillation when simultaneously monitoring the same field. Using contemporaneous meteorological data, we find that higher wind speeds at the tropopause correlate with a decrease in long-exposure ($t=10$ s) scintillation. Hence the winter months between June and August provide the best conditions for high precision photometry of bright stars at the Paranal Observatory. This work demonstrates that NGTS photometric data, collected for searching for exoplanets, contains within it a record of the scintillation conditions at Paranal.

==> sections/analysis/zold_longexp.tex <==
Figure~\ref{fig:ngts_ecmwf_1y} shows the annual variation in the NGTS \Cy\ measurements and the mean wind speed above Paranal, as computed from ECMWF data. The \Cy\ values for each sub-action as described in Section~\ref{sec:camvar} are displayed as light grey points. For each month we then compute the mean value and standard deviation. ECMWF data are acquired as monthly-averaged data from January 2016 through until April 2021. The mean of the full 4-5 years for each month is plotted, with corresponding standard deviation.

\begin{figure}
    \includegraphics[width=\columnwidth]{figures/1406_ngts_ecmwf_1y.pdf}
    \caption{\textit{Top panel}: NGTS measurements of \Cy\ folded onto a one-year period. Light grey points are the measurements for each sub-action and black circles show the mean for each month, with standard deviation shown as grey errorbars. \textit{Bottom panel}: ECMWF data for mean wind speed at 250\,hPa above Paranal. Faint blue points are the values for each month since 2016, blue circles are the mean values for each month across the full dataset with standard deviation shown as light blue errorbars.}
    \label{fig:ngts_ecmwf_1y}
\end{figure}

We can see that the NGTS measurements of \Cy, which acts as a proxy for the long-exposure scintillation index from Equation~\ref{eq:LE_prop}, shows a minima in the months of June to August. The ECMWF wind speed measurements peak in these months. This indicates that long-exposure scintillation does indeed decrease in the southern hemisphere months of June and August, when the wind speeds in the upper atmosphere are higher. This is because the higher wind speed averages out the turbulence cells passing across the line-of-sight of the telescope during the long exposure time. This causes an averaging out of the variation of light intensity and therefore reduces scintillation. This is governed in Equation~\ref{eq:LE_prop} as the $\frac{1}{V_{\perp}}$ term. We calculate a correlation coefficient of $-0.65,$ indicating moderately strong negative correlation between long-exposure scintillation and the mean wind speed.

\citet{Kornilov2012A&A...546A..41K} determined that long-exposure scintillation is minimal from May to September. Our conclusion is consistent with this. We also show the anti-correlation with high-altitude wind speed which is predicted by \citet{Kornilov2012A&A...546A..41K}.

==> sections/analysis/zold_shortexp.tex <==
Figure~\ref{fig:mass_ecmwf_1y} shows the annual changes in the scintillation index measured by the MASS from April 2016 to March 2021. We do note that the MASS data coverage is not uniform over these time periods due to operational interruptions. The ECMWF panel from Figure~\ref{fig:ngts_ecmwf_1y} is included to make comparison more simple.

\begin{figure}
    \includegraphics[width=\columnwidth]{figures/1406_mass_ecmwf_1y.pdf}
    \caption{\textit{Top panel}: MASS measurements of the scintillation index. Faint red points are the mean measurements of $\sigma_A$ for each night (04/2016-03/2021), red circles show the monthly mean with standard deviation shown as light red errorbars. \textit{Bottom panel}: Same as bottom panel in Figure~\ref{fig:ngts_ecmwf_1y}}
    \label{fig:mass_ecmwf_1y}
\end{figure}

It is evident from the top panel of Figure~\ref{fig:mass_ecmwf_1y} that the short-exposure scintillation index increases in the months of April to July. Additionally, the standard deviation, which indicates the variation in scintillation during the month, is much greater in these months. This suggests that scintillation conditions are much more unstable at the \PAR\ during these months. The peak in scintillation correlates with the peak in the high-altitude wind speeds measured by the ECMWF data. The higher wind speeds cause greater amounts of turbulence, therefore increasing $C_n^2(h)$. Meanwhile the short exposure time of the MASS measurements means that the averaging of the variation that occurs in the long-exposure regime is not a factor, consistent with the lack of a wind speed term in Equation~\ref{eq:SIseOsb}. This increases the mean scintillation during these months. The instability in scintillation conditions is likely due to higher wind speeds being more likely but less sustainable during these months \citep{ArcherJetstream}. We calculate a correlation coefficient of 0.86, indicating strong positive correlation between the MASS scintillation measurements and the mean wind speed.

It was found by \citet{Kornilov2012A&A...546A..41K} that in the southern hemisphere the short-exposure scintillation is maximal in the period from July to September. We find a similar result however the peak is closer to being from May to July. We also show the increase in short-exposure scintillation does correlate with wind speed, as predicted by \citet{Kornilov2012A&A...546A..41K}.

\Cref{fig:ngts_ecmwf_1y,fig:mass_ecmwf_1y} also support their conclusions that the seasonal variability does not exceed the quartiles (or in our case standard deviations) which indicates there is a reasonable probability of both good and poor conditions for bright star photometry year-round \citep{Kornilov2012A&A...546A..41K}.

==> sections/modelling.tex <==
The fractional amplitude of photometric noise due to scintillation (\sigY) can be estimated using the modified Young's approximation \citep{Young1967AJ.....72..747Y,Osborn2015MNRAS.452.1707O},

\begin{equation}\label{eq:modyoung}
   \sigYmath^2 = 10 \times 10^{-6} \CyMath^{2} D^{-4/3} t^{-1} (\sec z)^{3} \exp{(-2 h_{\text{obs}}/H)},
\end{equation}
where $D$ is the diameter of the telescope aperture (m), $t$ is exposure time used (s), $h_{\text{obs}}$ is the altitude of the observatory (2440\,m for Paranal), $H$ is the scale height of the atmospheric turbulence, taken to be 8000\,m. $z$ is the zenith distance, and therefore $\sec z$ approximates airmass. \Cy\ (m$^{2/3}$s$^{1/2}$) is the empirical coefficient.

This equation is taken from \citet{Osborn2015MNRAS.452.1707O}, where they introduced the empirical coefficient, \Cy, to improve the original approximation from \citet{Young1967AJ.....72..747Y}. This \Cy\ is typically found to be around $1.5$ for different sites, however this is a median value and the actual value can vary significantly across even a single night of observing \citep{Osborn2015MNRAS.452.1707O}. The median measured value of \Cy\ at the \PAR\ is $1.56^{+0.34}_{-0.29},$ where the limits are the upper and lower quartiles. This value is taken from \citet{Osborn2015MNRAS.452.1707O} where they extracted the results from data presented in \citet{Kornilov2012A&A...546A..41K}, where the authors originally identified that the Young's approximation underestimated scintillation by around 1.5 for most observing sites.

A more comprehensive measure of the scintillation index can be achieved using turbulence and wind velocity profilers. There exists two different scintillation regimes dependent on exposure tie of the observations. In the long-exposure regime ($t \gtrsim 0.1$\,s), the intensity speckles which cause scintillation traverse the telescope pupil and scintillation reduces due to temporal averaging, with a dependency on high-altitude wind speed. In the short-exposure regime, this averaging does not occur \citep{Osborn2015MNRAS.452.1707O}. NGTS uses 10 second exposures and so operates in the long-exposure regime. The long-exposure scintillation index is given by Equation~4 in \citet{Osborn2015MNRAS.452.1707O}, it has the form
\begin{equation}\label{eq:LE_prop}
    \sigma_{I,\text{le}}^2 \propto \int_{0}^{\infty} \frac{h^2 C_n^2(h)}{V_\perp (h)} \text{d}h,
\end{equation}
where $C_n^2(h)$ is the profile of the refractive index structure constant, h is the altitude of the turbulent layer, $V_\perp (h)$ is the wind velocity profile. The $h^2$ term demonstrates that high altitude turbulence has a greater effect on scintillation as scintillation is a propagation effect \citep{Osborn2015MNRAS.452.1707O}. The short-exposure scintillation index, Equation~3 in \citet{Osborn2015MNRAS.452.1707O}, does not have a wind velocity term. In this paper, we investigate whether there exists a seasonal correlation between wind speed and the long-exposure scintillation measurements, as predicted in \citet{Kornilov2012A&A...546A..41K}.

% A more comprehensive measure of the scintillation index can be achieved using vertical profiles of the refractive index structure constant of the atmosphere, $C_n^2(h),$ and the wind velocity. The exposure time of the observations can cause differences in the level of scintillation measured and therefore we use different equations to model this. For short-exposure observations, there is no temporal averaging of the intensity speckles that cause scintillation. In the long-exposure regime, the intensity speckles traverse the telescope pupil and scintillation reduces due to temporal averaging, with a dependency on high-altitude wind speed \citep{Osborn2015MNRAS.452.1707O}. The crossover between the short-exposure and long-exposure regimes is determined to be approximately 0.01-0.1\,s by \citet{Osborn2015MNRAS.452.1707O}, although this will depend on telescope diameter, airmass, wind direction and the wind velocity profile. This is evident from Equations~\ref{eq:SIleOsb} and~\ref{eq:SIseOsb} which follow. NGTS uses 10 second exposures and so operates in the long-exposure regime, thus if turbulence profilers were active at Paranal consistently then we could use the following equation given by \citet{Kenyon2006PASP..118..924K,Osborn2015MNRAS.452.1707O},

% \begin{equation}\label{eq:SIleOsb}
%     \sigma_{I,\text{le}}^2 = 10.66D^{-4/3} t^{-1} (\sec z)^{\alpha} \int_{0}^{\infty} \frac{h^2 C_n^2(h)}{V_\perp (h)} \text{d}h,
% \end{equation}
% where $C_n^2(h)$ is the profile of the refractive index structure constant, h is the altitude of the turbulent layer, $V_\perp (h)$ is the wind velocity profile and $\alpha$ is the exponent of the airmass which varies between $3$ for wind transverse to the azimuthal angle of the star, and $4$ for longitudinal wind. The $h^2$ term in the integral of this equation demonstrates that turbulence at higher altitudes has a greater effect on the scintillation measured by a telescope. The magnitude of the intensity speckles is directly linked to the propagation distance of the distorted wavefront from the turbulent layer. The further the light propagates, the more it can interfere with itself \citep{ThesisOsborn}. Therefore, higher altitude turbulence is usually the primary cause of scintillation and it is not dominated simply by the strongest turbulent layer of the atmosphere that is typically the layer nearest the ground \citep{Osborn2015MNRAS.452.1707O}.

% The Multi-Aperture Scintillation Sensor (MASS)-Differential Image Motion Montior (DIMM) instruments \citep{Kornilov2007MNRAS.382.1268K} use a short exposure of around 1\,ms to measure the intensity variation and derive scintillation indices. This is in the short-exposure scintillation regime. If provided with a turbulence profile, the short-exposure scintillation index is calculated as,

% \begin{equation}\label{eq:SIseOsb}
%     \sigma_{I,\text{se}}^2 = 17.34D^{-7/3} (\sec z)^{3} \int_{0}^{\infty} h^2 C_n^2(h) \text{d}h.
% \end{equation}

% MASS-DIMM data are available every night although we do not directly implement the above equation as the ESO portal\footnote{\url{http://archive.eso.org/wdb/wdb/asm/mass_paranal/form}} provides scintillation indices directly. It has been demonstrated that at sites such as Paranal, the long-exposure scintillation index, $\sigma_{I,\text{le}}$, is minimal between May and September, meanwhile the short-exposure scintillation index, $\sigma_{I,\text{se}}$, is maximal during this period \citep{Kornilov2012A&A...546A..41K}. In this paper, we investigate whether there exists a similar seasonal dependence in the scintillation measurements made with NGTS.
